Induction and Co-induction in Sequent Calculus

Proof search has been used to specify a wide range of computation systems. In order to build a framework for reasoning about such specifications, we make use of a sequent calculus involving induction and co-induction. These proof principles are based on a proof theoretic (rather than set-theoretic) notion of definition. Definitions are akin to (stratified) logic programs, where the left and right rules for defined atoms allow one to view theories as "closed" or defining fixed points. The use of definitions makes it possible to reason intensionally about syntax, in particular enforcing free equality via unification. We add in a consistent way rules for pre and post fixed points, thus allowing the user to reason inductively and co-inductively about properties of computational system making full use of higher-order abstract syntax. Consistency is guaranteed via cut-elimination, where we give the first, to our knowledge, cut-elimination procedure in the presence of general inductive and co-inductive definitions.

==> saturated.tex <==
\newpage
\def\RED{{\hbox{\bf RED}}}
\section{An alternative cut elimination (work in progress)}

\subsection{Normalizability}

To show the termination of cut-reduction, we define two orderings on 
derivations: {\em normalizability} and {\em reducibility} 
(called computability in~\cite{martin-lof71sls}).  
The well-foundedness of the normalizability ordering immediately
implies that the cut-elimination process terminates. 
Reducibility is a superset of normalizability 
and hence its well-foundedness implies the well-foundedness of 
normalizability. 
The usual proof technique with reducibility (in sequent calculus)
is to show that all derivations in $\Linc$ are reducible, 
and hence normalizable. However, in the presence of co-induction,
we need to form certain closure of reducible derivations, which
we refer to as {\em saturated sets}. We shall show that the
set of all derivations is included in all saturated sets, hence
all derivations are reducible. 

\begin{definition}
\label{def:norm}
We define the set of {\em normalizable} derivations to be the smallest
set that satisfies the following conditions:
\begin{enumerate}
\item
If a derivation $\Pi$ ends with a multicut, then it is normalizable
if every reduct of $\Pi$ is normalizable.

\item If a derivation $\Pi$ ends with $\coindR$:
$$
\infer[\coindR]
{\Seq \Gamma {p\bar t}}
{
\deduce{\Seq \Gamma {S\bar t}}{\Pi'}
&
\deduce{\Seq {S \bar x}{B\,S\,\bar x}}{\Pi_S}
}
$$
then $\Pi$ is normalizable if $\Pi'$ and $\Pi_S$ are normalizable,
and for every derivation $\Xi$ of $\Seq \Delta {S\,\bar u}$,
the derivation
$$
\infer[\mc]
{\Seq \Delta {B\,S\,\bar u}}
{
  \deduce{\Seq \Delta {S\,\bar u}}{\Pi'}
&
  \deduce{\Seq {S\,\bar u} {B\,S\,\bar u}}{\Pi_S[\bar u/ \bar x]}
}
$$
is normalizable.

\item
If a derivation ends with any rule other than a multicut and $\coindR$,
then it is normalizable if the premise derivations are normalizable.
\end{enumerate}
These clauses assert that a given derivation is normalizable
provided certain (perhaps infinitely many) other derivations are
normalizable.
If we call these other derivations the predecessors of the given
derivation, then a derivation is normalizable if and only if the tree
of the derivation and its successive predecessors is well-founded.
In this case, the well-founded tree is called the {\em normalization} of
the derivation.

The set of all normalizable derivations is denoted by $\aleph$.
\end{definition}

Since a normalization is well-founded, it has an associated induction
principle:  for any property $P$ of derivations, if for every
derivation $\Pi$ in the normalization, $P$ holds for every predecessor
of $\Pi$ implies that $P$ holds for $\Pi$, then $P$ holds for every
derivation in the normalization.

\begin{lemma}
\label{lm:norm-cut-free}
If there is a normalizable derivation of a sequent, then there is a
cut-free derivation of the sequent.
\end{lemma}
\begin{proof}  Let $\Pi$ be a normalizable derivation of the sequent
$\Seq{\Gamma}{\Bscr}$.
We show by induction on the normalization of $\Pi$ that there is a
cut-free derivation of $\Seq{\Gamma}{\Bscr}$.
\begin{enumerate}

\item
If $\Pi$ ends with a multicut, then any of its reducts is one of its
predecessors  and so is normalizable.
But the reduct is also a derivation of $\Seq{\Gamma}{\Bscr}$, so by the
induction hypothesis this sequent has a cut-free derivation.

\item
Suppose $\Pi$ ends with a rule other than multicut.
Since we are given that $\Pi$ is normalizable, by definition the
premise derivations are normalizable.
These premise derivations are the predecessors of $\Pi$, so by the
induction hypothesis there are cut-free derivations of the premises.
Thus there is a cut-free derivation of $\Seq{\Gamma}{\Bscr}$.
\end{enumerate}
\qed
\end{proof}

The next lemma states that normalization is closed under
substitutions.


\begin{lemma}
\label{lm:subst-norm}
If $\Pi$ is a normalizable derivation, then for any substitution
$\theta$, $\Pi\theta$ is normalizable.
\end{lemma}
\begin{proof} We prove this lemma by induction on the normalization of
$\Pi$.
\begin{enumerate}
 
\item
If $\Pi$ ends with a multicut, then $\Pi\theta$ also ends with a
multicut. By Lemma~\ref{lm:reduct subst} every reduct of
$\Pi\theta$ corresponds to a reduct of $\Pi$, therefore by
induction hypothesis every reduct of $\Pi\theta$ is normalizable,
and hence $\Pi\theta$ is normalizable.
 
\item
Suppose $\Pi$ ends with a rule other than multicut and has premise
derivations $\{\Pi_i\}$.
By Definition~\ref{def:subst} each premise derivation in
$\Pi\theta$ is either $\Pi_i$ or $\Pi_i\theta$.
Since $\Pi$ is normalizable, $\Pi_i$ is normalizable, and so by the
induction hypothesis $\Pi_i\theta$ is also normalizable.
Thus $\Pi\theta$ is normalizable.
\qed
\end{enumerate}
\end{proof}

\subsection{Saturated sets}

We say that a set of derivations $\Rscr$ is closed under substitution
if $\Pi \in \Rscr$ implies $\Pi\theta \in \Rscr$ for every substitution $\theta.$

\begin{definition}
A set $\Rscr$ of normalizable derivations is {\em saturated} 
if it is closed under substitution and the following hold for every derivation $\Pi$:
\begin{enumerate}
\item If $\Pi$ ends with $\mc$ then $\Pi \in \Rscr$ if and only if
all its reducts are in $\Rscr.$
\item If $\Pi$ ends with $\oimpR$:
$$
\infer[\oimpR]
{\Seq \Gamma {B \oimp C}}
{\deduce{\Seq {\Gamma,B } C}{\Pi'}}
$$
then $\Pi \in \Rscr$ if and only if $\Pi' \in \Rscr$ and
for every substitution $\theta$ and every derivation $\Xi \in \Rscr$ of
the sequent $\Seq{\Delta}{B\theta},$ the derivation
$$
\infer[mc]
{\Seq{\Delta, \Gamma\theta}{C\theta}}
{
\deduce{\Seq{\Delta}{B\theta}}{\Xi}
&
\deduce{\Seq{\Gamma\theta, B\theta}{C\theta}}{\Pi'\theta}
}
$$
is in $\Rscr.$

\item
If $\Pi$ ends with the $\oimpL$ rule or the $\indL$
rule, then $\Pi \in \Rscr$ if and only if the right premise
derivation is in $\Rscr$ and the other premise derivation
is normalizable.

\item If $\Pi$ ends with $\coindR$ rule:
$$
\infer[\coindR]
{\Seq \Gamma {p\bar t}}
{
\deduce{\Seq \Gamma {S\bar t}}{\Pi'}
&
\deduce{\Seq {S \bar x}{B\,S\,\bar x}}{\Pi_S}
}
$$
then $\Pi \in \Rscr$ if and only if $\Pi', \Pi_S  \in \Rscr$,
and for every derivation $\Xi \in \Rscr$ of 
$\Seq \Delta {S\bar u}$,
the derivation
$$
\infer[\mc]
{\Seq {\Delta}{B\,S\,\bar u}}
{
\deduce{\Seq \Delta {S\,\bar u}}{\Xi}
&
\deduce{\Seq {S\,\bar u}{B\,S\,\bar u}}{\Pi_S[\bar u/ \bar x]}
}
$$
is in $\Rscr.$

\item
If the derivation ends with any other rule, with the premise derivations
$\{ \Pi_k \}_{k \in I}$ for some index set $I$, then $\Pi \in \Rscr$ if and only if 
$\Pi_k \in \Rscr$ for every $k \in I.$
\end{enumerate}
\end{definition}

Note that since every saturated set is a subset of the set of reducible derivations,
all its elements are ordered by the well-founded reducibility ordering.

\subsection{Reducibility}

The definition of reducibility is by induction on the level 
of the derivation: 
in the definition of reducibility for derivations of level $i$
we assume that reducibility is already defined for all levels
$j < i$. 
(Recall from Definition~\ref{def:level} that the level of a derivation
is defined to be the level of the consequent of its end-sequent.)
We shall denote the set of all reducible derivations with $\Re$.
The notation $\Re_i$ denotes the set of all reducible derivations of level $i$,
while $\Re_{< i}$ ($\Re_{\leq i}$) denotes the set of reducible derivations of level
smaller than $i$ (respectively, smaller or equal to $i$).
In the following definition, we refer to a derivation $\Pi$ as an $i$-level derivation if
$\level{\Pi} = i$.

\begin{definition}
\label{def:comp}
For any $i$, we define the set of {\em reducible} $i$-level
derivations to be the smallest set of $i$-level derivations that
satisfies the following conditions:
\begin{enumerate}
\item
If an $i$-level derivation $\Pi$ ends with a multicut, then it is $i$-reducible if
every reduct of $\Pi$ is $i$-reducible.

\item
Suppose the $i$-level derivation $\Pi$ ends with the implication right rule
\begin{displaymath}
\infer[\oimpR]{\Seq{\Gamma}{B \oimp C}}
	{\deduce{\Seq{B,\Gamma}{C}}
		{\Pi'}}
\enspace .
\end{displaymath}
Let $j$ be the level of $B$ and let $k$ be the level of $C$. 
Then the derivation is $i$-reducible if the premise
derivation $\Pi'$ is $k$-reducible and, for every substitution
$\theta$, multiset $\Delta$ of formulas, and $j$-reducible
derivation $\Pi''$ of $\Seq{\Delta}{B\theta}$, the derivation
\begin{displaymath}
\infer[\mc]{\Seq{\Delta,\Gamma\theta}{C\theta}}
	{\deduce{\Seq{\Delta}{B\theta}}
		{\Pi''}
	& \quad 
	& \deduce{\Seq{B\theta,\Gamma\theta}
	       {C\theta}}
		{\Pi'\theta}}
\end{displaymath}
is $k$-reducible.

\item
If the derivation ends with the $\oimpL$ rule or the $\indL$
rule, then it is $i$-reducible if the right premise
derivation is $i$-reducible and the other premise derivations
are normalizable.

\item If $\Pi$ ends with $\coindR$ rule:
$$
\infer[\coindR]
{\Seq \Gamma {p\,\bar t}}
{
\deduce{\Seq \Gamma {S\,\bar t}}{\Pi'}
&
\deduce{\Seq {S\,\bar x}{B\,S\,\bar x}}{\Pi_S}
}
$$
then it is reducible if for every saturated set $\Rscr$,
$\Pi', \Pi_S \in \Rscr$ and for every derivation $\Xi$ of $\Seq \Delta {S\,\bar u}$
in $\Rscr$, the derivation
$$
\infer[mc]
{\Seq \Delta {B \, S\,\bar u}}
{
\deduce{\Seq \Delta {S\,\bar u}}{\Xi}
&
\deduce{\Seq {S\,\bar x}{B\,S\,\bar u}}{\Pi_S[\bar u/ \bar u]}
}
$$
is also in $\Rscr.$

\item
If the derivation ends with any other rule, with the premise derivations
$\{ \Pi_k \}_{k \in I}$ for some index set $I$, then it is
$i$-reducible if every derivation $\Pi_k$ is 
$\level{\Pi_k}$-reducible.
\end{enumerate}

These clauses assert that a given derivation is reducible
provided certain (perhaps infinitely many) other derivations are
reducible.
If we call these other derivations the predecessors of the given
derivation, then a derivation is reducible only if the tree of
the derivation and its successive predecessors is well-founded.
In this case, the well-founded tree is called the {\em reduction} of
the derivation.  
\end{definition}

In defining reducibility for a derivation of (writing the signatures explicitly)
$$\Seq{\Gamma}{B \oimp C}$$
ending with $\oimpR$ we quantify over reducible derivations of
$$\Seq{\Delta}{B\theta}.$$
This is legitimate since we are defining reducibility for a
derivation having level $\max(\level{B}+1,\level{C})$, so the set of
reducible derivations having level $\level{B}$ is
already defined (substitution does not change the level).

For a derivation ending with $\oimpL$, $\indL$ or $\coindR$,
some premise derivations may have consequents with a higher level than
that of the consequent of the conclusion.
As a result, we cannot use the reducibility of those premise
derivations to define the reducibility of the derivation as a whole,
since the reducibility of the premise derivations may not yet be
defined. 
Thus we use the weaker notion of normalizability for those premise
derivations.

From now on, we shall refer to an $i$-reducible derivation, for some level $i$,
as simply reducible derivation. We denote with $\RED$ the set of all
reducible derivations.

\begin{lemma}
\label{lm:comp-norm}
If a derivation is reducible, then it is normalizable.
\end{lemma}
\begin{proof}
By induction on the reduction tree and Definition~\ref{def:norm} (normalizability).
\qed
\end{proof}

\begin{lemma}
\label{lm:subst-comp}
If $\,\Pi$ is a reducible derivation, then for any substitution
$\theta$, $\Pi\theta$ is reducible.
\end{lemma}
\begin{proof}
We prove this lemma by induction on the reduction of $\Pi$.
\begin{enumerate}

\item
If $\Pi$ ends with a multicut, then $\Pi\theta$ also ends with a
multicut. By Lemma~\ref{lm:reduct subst} every reduct of 
$\Pi\theta$ is an instance of a reduct of $\Pi$. Hence by induction
hypothesis all reducts of $\Pi\theta$ are reducible.

\item
If $\Pi$ ends with the implication right rule then $\Pi$ and
$\Pi\theta$ are
\begin{displaymath}
\infer[\oimpR]{\Seq{\Gamma}{B \oimp C}}
	{\deduce{\Seq{B,\Gamma}{C}}
		{\Pi'}}
\qquad\qquad
\infer[\oimpR]{\Seq{\Gamma\theta}
                  {(B \oimp C)\theta}}
	{\deduce{\Seq{B\theta,\Gamma\theta}
	        {C\theta}}
		{\Pi'\theta}}
\enspace .
\end{displaymath}
$\Pi\theta$ is reducible if $\Pi'\theta$ is reducible and, for every
substitution $\theta'$, multiset $\Delta$, and reducible derivation
$\Pi''$, the derivation $\Xi$
\begin{displaymath}
\infer[\mc]{\Seq{\Delta,\Gamma\theta\theta'}
		{C\theta\theta'}}
	{\deduce{\Seq{\Delta}{B\theta\theta'}}
		{\Pi''}
	& \quad 
	& \deduce{\Seq{B\theta\theta',\Gamma\theta\theta'}
			{C\theta\theta'}}
		{\Pi'\theta\theta'}}
\end{displaymath}
is also reducible.
$\Pi'\theta$ is reducible by the induction hypothesis, and
$\Xi$ is reducible since it is a predecessor of $\Pi$.
Therefore $\Pi\theta$ is reducible.

\item
If $\Pi$ ends with $\oimpL$ or $\indL$, then the right premise
derivation is reducible and the other premise derivations are
normalizable.
By Definition~\ref{def:subst} each premise derivation in
$\Pi\theta$ is obtained by applying $\theta$ to a premise derivation
in $\Pi$.
By the induction hypothesis the right premise derivation of
$\Pi\theta$ is reducible, and by Lemma~\ref{lm:subst-norm} the other
premise derivations are normalizable.
Thus $\Pi\theta$ is reducible.

\item Suppose $\Pi$ ends with $\coindR$,  
$$
\infer[\coindR]
{\Seq{\Delta}{p\,\bar{t}}}
{
  \deduce{\Seq{\Delta}{S\,\bar{t}}}{\Pi'}
  &
  \deduce{\Seq{S\,\bar{x}}{D\,S\,\bar{x}}}{\Pi_S} 
}
$$
where $p\,\bar{x} \defnu D\,p\,\bar{x}$.
Then by definition, $\Pi'$ and $\Pi_S$ are normalizable.
The derivation $\Pi\theta$ is
$$
\infer[\coindR \enspace .]
{\Seq{\Delta\theta}{(p\,\bar{t})\theta}}
{
  \deduce{\Seq{\Delta}{(S\,\bar{t})\theta}}{\Pi'\theta}
  &
  \deduce{\Seq{S\,\bar{x}}{D\,S\,\bar{x}}}{\Pi_S} 
}
$$
Since normalizability is closed under substitution (Lemma~\ref{lm:subst-norm}),
it follows that $\Pi'\theta$ is reducible, hence $\Pi\theta$ is reducible.

\item
Suppose $\Pi$ ends with any other rule and has premise
derivations $\{\Pi_i\}$.
By Definition~\ref{def:subst} each premise derivation in
$\Pi\theta$ is either $\Pi_i$ or $\Pi_i\theta$.
Since $\Pi$ is reducible, $\Pi_i$ is reducible, and so by the
induction hypothesis $\Pi_i\theta$ is also reducible.
Thus $\Pi\theta$ is reducible.
\qed
\end{enumerate}
\end{proof}



